A Generic Approach for Reproducible Model Distillation

Model distillation has been a popular method for producing interpretable machine learning. It uses an interpretable "student" model to mimic the predictions made by the black box "teacher" model. However, when the student model is sensitive to the variability of the data sets used for training even when keeping the teacher fixed, the corresponded interpretation is not reliable. Existing strategies stabilize model distillation by checking whether a large enough corpus of pseudo-data is generated to reliably reproduce student models, but methods to do so have so far been developed for a specific student model. In this paper, we develop a generic approach for stable model distillation based on central limit theorem for the average loss. We start with a collection of candidate student models and search for candidates that reasonably agree with the teacher. Then we construct a multiple testing framework to select a corpus size such that the consistent student model would be selected under different pseudo samples. We demonstrate the application of our proposed approach on three commonly used intelligible models: decision trees, falling rule lists and symbolic regression. Finally, we conduct simulation experiments on Mammographic Mass and Breast Cancer datasets and illustrate the testing procedure throughout a theoretical analysis with Markov process. The code is publicly available at https://github.com/yunzhe-zhou/GenericDistillation.

==> Generic Distillation (Nature ML)/cover-letter.tex <==
% !TEX program = pdflatex
\input{cover_letter_template}

\begin{document}
\hfill{\today}

Nature Machine Intelligence

\bigskip

Dear Editors:

We are writing to submit our manuscript ``A Generic Approach for Reproducible Model Distillation'' to the \emph{Nature Machine Intelligence}.

Model distillation is a common procedure in interpretable Machine Learning, which re-represents the ``black-box'' outputs of Machine Learning algorithms in terms of simpler, usually structured models incorporating a search over structure. This is often described as a black-box ``teacher'' training an interpretable ``student'' with decision trees being the most common student models, but other explanation systems such as LIME can also be placed in this framework. 

An important concern in this framework is the reproducibility of the distillation process, with a few papers showing that the process of training decision trees and LIME require a significantly larger number of samples than is usually employed to reliably produce the same explanation. This paper extends these to a generic class of structured student models, including decision trees, falling rule lists, and symbolic regression and presents the means to both assess the reproducibility of the resulting student and estimate how much additional computing would be needed to provide reproducibility guarantees. 


We have not had any prior discussions about the work described in the manuscript with an editor from Nature Machine Intelligence, and there are no related manuscripts currently under consideration or in press elsewhere.

Given the increasing interest in interpretable machine learning per se, and the increasing use of model distillation, we believe this will be of genuine interest to the readers of Nature Machine Intelligence. 



% This paper extends our work of \red{Conference Paper} by addressing \red{X, Y, and Z additional points}.

% We suggest the following action editors and referees for our submission. Please note conflicts of interest with action editors Killian Weinberger, Michael Mahoney and Boaz Nadler. 

% Action Editors
% \begin{itemize}
%     \item Genevera Allen, Rice University (gallen@rice.edu)
%     \item Miguel Carreira-Perpinan, UC Merced (mcarreira-perpinan@ucmerced.edu)
%     \item Adrian Weller, University of Cambridge (adrian.weller@eng.cam.ac.uk)
%     \item Maya Gupta, University of Washington (gupta@ee.washington.edu)
%     \item Pradeep Ravikumar, Carnegie Mellon University (pradeepr@cs.cmu.edu)
% \end{itemize}

% Reviewers:
% \begin{itemize}
%     \item Cynthia Rudin, Duke University (cynthia@cs.duke.edu)
%     \item Aaron Fisher, Foundation Medicine (afishe27@alumni.jh.edu)
%     \item Jack Dunn, Interpretable AI (jack.dunn.nz@gmail)
%     \item Alexandra Chouldechova, Carnegie Mellon University (achould@cmu.edu)
% \end{itemize}

% Our submission has the following keywords: Interpretability,  Model Distillation, Multiple Testing, Explainable Artificial Intelligence, Reproducibility

% As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Yunzhe Zhou (University of California, Berkeley)\\
Peiru Xu (University of California, Berkeley)\\
Giles Hooker (University of California, Berkeley)

\end{document}








































==> cover-letter.tex <==
% !TEX program = pdflatex
\input{cover_letter_template}

\begin{document}
\hfill{\today}

Nature Machine Intelligence

\bigskip

Dear Editors:

We are writing to submit our manuscript ``A Generic Approach for Reproducible Model Distillation'' to the \emph{Nature Machine Intelligence}.

Model distillation is a common procedure in interpretable Machine Learning, which re-represents the ``black-box'' outputs of Machine Learning algorithms in terms of simpler, usually structured models incorporating a search over structure. This is often described as a black-box ``teacher'' training an interpretable ``student'' with decision trees being the most common student models, but other explanation systems such as LIME can also be placed in this framework. 

An important concern in this framework is the reproducibility of the distillation process, with a few papers showing that the process of training decision trees and LIME require a significantly larger number of samples than is usually employed to reliably produce the same explanation. This paper extends these to a generic class of structured student models, including decision trees, falling rule lists, and symbolic regression and presents the means to both assess the reproducibility of the resulting student and estimate how much additional computing would be needed to provide reproducibility guarantees. 


We have not had any prior discussions about the work described in the manuscript with an editor from Nature Machine Intelligence, and there are no related manuscripts currently under consideration or in press elsewhere.

Given the increasing interest in interpretable machine learning per se, and the increasing use of model distillation, we believe this will be of genuine interest to the readers of Nature Machine Intelligence. 



% This paper extends our work of \red{Conference Paper} by addressing \red{X, Y, and Z additional points}.

% We suggest the following action editors and referees for our submission. Please note conflicts of interest with action editors Killian Weinberger, Michael Mahoney and Boaz Nadler. 

% Action Editors
% \begin{itemize}
%     \item Genevera Allen, Rice University (gallen@rice.edu)
%     \item Miguel Carreira-Perpinan, UC Merced (mcarreira-perpinan@ucmerced.edu)
%     \item Adrian Weller, University of Cambridge (adrian.weller@eng.cam.ac.uk)
%     \item Maya Gupta, University of Washington (gupta@ee.washington.edu)
%     \item Pradeep Ravikumar, Carnegie Mellon University (pradeepr@cs.cmu.edu)
% \end{itemize}

% Reviewers:
% \begin{itemize}
%     \item Cynthia Rudin, Duke University (cynthia@cs.duke.edu)
%     \item Aaron Fisher, Foundation Medicine (afishe27@alumni.jh.edu)
%     \item Jack Dunn, Interpretable AI (jack.dunn.nz@gmail)
%     \item Alexandra Chouldechova, Carnegie Mellon University (achould@cmu.edu)
% \end{itemize}

% Our submission has the following keywords: Interpretability,  Model Distillation, Multiple Testing, Explainable Artificial Intelligence, Reproducibility

% As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

Yunzhe Zhou (University of California, Berkeley)\\
Peiru Xu (University of California, Berkeley)\\
Giles Hooker (University of California, Berkeley)

\end{document}







































